Unifying the Convergences in Multilingual Neural Machine Translation

Although all-in-one-model multilingual neural machine translation (multilingual NMT) has achieved remarkable progress, the convergence inconsistency in the joint training is ignored, i.e., different language pairs reaching convergence in different epochs. This leads to the trained MNMT model over-fitting low-resource language translations while under-fitting high-resource ones. In this paper, we propose a novel training strategy named LSSD (Language-Specific Self-Distillation), which can alleviate the convergence inconsistency and help MNMT models achieve the best performance on each language pair simultaneously. Specifically, LSSD picks up language-specific best checkpoints for each language pair to teach the current model on the fly. Furthermore, we systematically explore three sample-level manipulations of knowledge transferring. Experimental results on three datasets show that LSSD obtains consistent improvements towards all language pairs and achieves the state-of-the-art.

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/0_abstract.tex <==
\begin{abstract}
Although all-in-one-model multilingual neural machine translation (multilingual NMT) has achieved remarkable progress, the \textit{convergence inconsistency} in the joint training is ignored, \ie{different language pairs reaching convergence in different epochs}.
This leads to the trained MNMT model over-fitting low-resource language translations while under-fitting high-resource ones.
In this paper, we propose a novel training strategy named LSSD (\textbf{L}anguage-\textbf{S}pecific \textbf{S}elf-\textbf{D}istillation), which can alleviate the convergence inconsistency and help MNMT models achieve the best performance on each language pair simultaneously.
Specifically, LSSD picks up \textit{language-specific best checkpoints} for each language pair to teach the current model on the fly.
Furthermore, we systematically explore three sample-level manipulations of knowledge transferring. 
Experimental results on three datasets show that LSSD obtains consistent improvements towards all language pairs and achieves the state-of-the-art
\footnote{Our code is publicly available at \url{https://github.com/OrangeInSouth/LSSD}.}
. 
% Compared to the previous distillation-based method, our LSSD resolves the lack of improvement on low-resource language pairs.



%state-of-the-art performance.\footnote{We release our code in: \href{https://github.com/xxx/xxx}{https://github.com/xxx/xxx}}
\end{abstract}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/1_introduction.tex <==
\section{Introduction}
\begin{figure}[ht]
  \centering
    \includegraphics[clip,width=1.0\columnwidth,]{figure/Convergence_Inconsistency.pdf}
    \caption{Loss curves of a multilingual NMT model trained to translate 4 languages into English. The upper two boxes illustrate low-resource directions. And the high-resource ones are placed in the bottom part. The x-axis and y-axis indicate training epochs and dev losses respectively. Dotted lines mark language-specific best checkpoints (colorful ones) as well as the overall best checkpoint (the black one).}
  \label{fig:case}
\end{figure}
% 第一段：NMT => MNMT
Neural machine translation (NMT)~\cite{kalchbrenner-blunsom-2013-recurrent,sutskever-etal-2014-sequence} has witnessed enormous and significant progress, including network structures~\cite{cho-etal-2014-learning,bahdanau-etal-2015-neural,gehring-etal-2017-convolutional,vaswani-etal-2017-attention}, attention mechanism~\cite{luong-etal-2015-effective,liu-etal-2016-neural,shen-etal-2018-disan} and decoding strategies~\cite{xia-etal-2017-deliberation,geng-etal-2018-adaptive,zhou-etal-2019-synchronous}.
While achieving promising performance~\cite{wu-etal-2016-googles,hassan-etal-2018-achieving}, widely-used {\em bilingual} NMT actually causes huge computational cost especially when tackling numerous language pairs, thereby facilitating the recent emergence of {\em multilingual} NMT~\cite{ha-etal-2016-toward,firat-etal-2016-multi,johnson-etal-2017-googles,lu-etal-2018-neural,aharoni-etal-2019-massively}. 
By directly translating multiple language pairs with one model, multilingual NMT~\cite{tan-etal-2018-multilingual,zhang-etal-2020-improving,fan-etal-2021-beyond,zhang-etal-2021-share} quadratically accelerates deployment and effectively encourages transfer learning between similar languages, which greatly benefits low-resource directions~\cite{arivazhagan-etal-2019-massively} and successfully enables zero-shot translation~\cite{gu-etal-2019-improved}.


% 第二段：Problem
Despite the remarkable success, multilingual NMT~\cite{liu-etal-2020-multilingual-denoising,lin-etal-2021-learning} clearly expresses a strong disagreement on the uniform convergence point across various translation corpora.
The underlying reason is the imbalance and heterogeneity of available data in multilingual training~\cite{wang-etal-2020-balancing,wu-etal-2021-uncertainty}, which also explains why the disagreement between high-resource languages (HRLs) and low-resource languages (LRLs) is more pronounced, as illustrated in Figure~\ref{fig:case}. 
Particularly, a fairly common and important observation about the learning of multilingual NMT is that
HRLs typically encounter underfitting, while extremely severe overfitting generally arises in LRLs. 

% 第三段：Motivation
In this paper, we cast this convergence inconsistency as the performance deficit between the multilingual NMT model and its own language-specific best checkpoints, and aim to reduce this deficit.
Towards tacking this problem, we propose a novel training strategy dubbed \textbf{L}anguage-\textbf{S}pecific \textbf{S}elf-\textbf{D}istillation (LSSD).
At each training step, LSSD appoints recent best checkpoints oriented to each language pair as teacher models and treats the current training model as the student learning from each teacher model in a knowledge distillation manner.
% In fact, LSSD ensures the progressiveness of teacher models with a dynamic teacher-updating mechanism, that is, once the student achieves better performance on a certain language pair, it would replace the corresponding teacher model.
% And since these teacher models are copied from generated checkpoints, our method avoids the overheads of training teacher models.
Differently depending on data selection and strength of performing knowledge distillation indeed, several practical strategies are employed to potentially provide a relatively fine-grained manipulation of knowledge transferring:
1) \textsc{LSSD-Whole}, which performs distillation on all data samples equally; 
2) \textsc{LSSD-Selective}, which selects samples for distillation conditioned on whether the teacher performs better than the student;
3) \textsc{LSSD-Adaptive}, which varies the distillation strength according to the sample-level performance ratio between the teacher and student.

% 第四段：实验
Experimental results on TED talks\footnote{\url{https://www.ted.com/participate/translate}} and WMT under {\em many-to-one} and {\em one-to-many} settings demonstrate that our method can obtain consistent and significant improvement through remedying the convergence inconsistency, ultimately achieving state-of-the-art translation performance.




==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/2_preliminaries.tex <==
\section{Preliminaries}
\subsection{Neural Machine Translation}
Bilingual neural machine translation (Bilingual NMT) translates a sentence $x$ in source language into a sentence $y$ in target language. Given a parallel corpus ${D} = \{(x,y) \in \mathcal{X} \times \mathcal{Y}\}$, the neural machine translation model is commonly trained with the Maximum Likelihood Estimation (MLE):
\begin{align}
\theta^* &= \argmax\limits_{\theta} \mathbb{E}_{(x,y) \sim {D}} \sum\limits_{i \le |y|} \log P(y_i | x,y_{<i}; \theta),
\label{eq:MLE_loss}
\end{align}
 where $P(\cdot|\cdot; \theta)$ is the conditional probability with model $\theta$, which is usually implemented in an encoder-decoder architecture~\citep{bahdanau-etal-2015-neural,vaswani-etal-2017-attention}.
 
\subsection{Multilingual Neural Machine Translation}
% Although NMT has been on par with human beings in single language pair translations, it is unaffordable to deploy one model for each language pair~\citep{xie-etal-2021-importance}.
% MNMT is proposed for alleviating the above problem and has attracted much attention in recent years. 
Multilingual neural machine translation (multilingual NMT) translates multiple language pairs with one unified model.
In this work, we follow \citet{johnson-etal-2017-googles} to train a multilingual NMT model jointly using training datasets of $L$ language pairs $D^{train}=\{D^{train}_1,...,D^{train}_l...,D^{train}_L\}$, where $D^{train}_l$ is the dataset of language pair $(S_l,T_l)$. 
To encode and decode diverse languages to/from a shared semantic space, a large multilingual vocabulary $\mathcal{V}$ is constructed.
And a language tag is appended to the beginning of source sentences to specify the target language.
% For example, the tag `2en' means translating any source language sentence to the English sentence.
Similar with bilingual NMT, the MNMT model is also trained with the same objective as Eq.\ref{eq:MLE_loss}.

\paragraph{Model Selection Strategy}
The common practice saves a checkpoint at the end of each training epoch, and evaluates its performance on a set of development sets $D^{dev}=\{D^{dev}_1,...,D^{dev}_l,...,D^{dev}_L\}$.
Finally the checkpoint with minimal average dev loss is selected as the \textit{overall best checkpoint}.
This average dev loss could be formalized as:
\begin{align}
\label{eq:dev loss}
    \mathcal{L}^{dev}(\theta, D^{dev})=\frac{1}{L}\sum\limits_{l=1}^{L}\mathcal{L}(D^{dev}_l;\theta).
\end{align}
% From Equation~\ref{eq:dev loss}, we can see that this average-based dev loss only reflects the overall performance while not performances on each individual language pair. 
In our work, we record language-specific dev losses $\mathcal{L}^{dev}_l$ and save the \textit{language-specific best checkpoint} towards each language pair $l$ additionally.

\begin{figure*}[t]
  \centering
    \includegraphics[clip,width=1.9\columnwidth,]{figure/LSSD_Razer.pdf}
    \caption{%Illustration of Language-Specific Self-Distillation (LSSD). 
    The upper part portrays the process of bilingual LSSD. The multilingual LSSD process is shown in the bottom part.
    The blue boxes indicates the student model (NMT Model or multilingual NMT model) and the inside value represents its dev loss in the current training epoch.
    The orange box indicates the teacher model and its loss means its dev loss in the corresponding training epoch.
    The distillation switch, which determines whether to perform distillation in the current epoch, is drawn as an ellipse with grey for off and green for on.}
  \label{fig:LSSD_example}
\end{figure*}

\subsection{Self-Distillation}
Knowledge distillation is an effective model compression technology that distills knowledge from a high-capacity teacher model into the compact student model~\citep{hinton2015distilling}. Self-distillation is an intriguing variation on knowledge distillation with the fundamental difference that self-distillation uses the same network for both the teacher and student model.~\citep{8953762,Zhang_2019_ICCV}.
\citet{8953762} use models in earlier epochs to guide the training of later epochs, which boosts the predictive accuracy in image classification by a large margin.
In this paper, we extend this idea to let the student model learn multiple different targets in the same training epoch and the number of targets is constantly changing in different epochs.


==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/3_method.tex <==
\section{Language-Specific Self-Distillation}
In this section, we first introduce the overall process of LSSD. 
Then, we provide a detailed formalization of LSSD, with special emphasis on the three fine-grained manipulations on knowledge transferring. 



\subsection{Overall} \label{subsection:LSSD}

In this subsection, we present an overview of our training strategy for multilingual NMT, as illustrated in Figure \ref{fig:LSSD_example}. 
Specifically, we first take bilingual self-distillation as an example to show the distillation learning process.
Then, we describe the multilingual self-distillation model and how it performs self-distillation towards multiple language pairs.

\paragraph{Bilingual LSSD}
Traditional bilingual neural machine translation builds a Sequence-to-Sequence model for training.
In our bilingual LSSD, we introduce an additional teacher model and a distillation switch.
The teacher model is used to guide the original machine translation model and the switch is designed to decide whether the teacher model is working or not in the current training epoch.
We depict the bilingual LSSD process in the upper half of Figure ~\ref{fig:LSSD_example}.

Normally, at the beginning of training, the loss monotonically decreases, and we refer to this process as ``initial training stage''. 
And $k'$ denotes the number of epochs the initial training stage lasts. It should be noted that the value of $k'$ is not a hyperparameter but is up to the training process.
During these $k'$ epochs, we do not perform distillation (keep the distillation switch off) but replace iteratively the teacher with the better-performance student which has a lower loss.
As we all know, the lower loss, the better. 
Therefore, if the teacher's loss is lower than the student's loss, we turn on the switch, as shown in the $k'$+1 epoch.
In fact, we do not perform distillation due to the switch being closed at the beginning of this epoch.
In the $k'$+2 epoch, since the switch is on, the teacher model distills the student model.
And since the teacher's loss is still lower than the student's loss, the switch remains on.
In the $k'$+3 epoch, the switch also shows turned on, the distillation learning is performed.
But the teacher's loss is higher than the student's loss, we turn off the switch.
At the same time, we replace the teacher model with the current student model to complete the teacher updating.




\paragraph{Multilingual LSSD}


Multilingual LSSD is a complex version of bilingual LSSD, which needs to maintain multiple language-specific teachers and conduct multi-objective distillation learning.
We illustrate the multilingual LSSD process in the bottom half of Figure~\ref{fig:LSSD_example}.
The blue box also means the student model (the current training MNMT model) and the value of loss represents the average loss of the student over multiple language-specific dev sets in the corresponding training epoch.
The different kinds of orange boxes represent different language-specific teacher models, and each loss means different language dev loss in the current training epoch.
For example, the darkest orange box \texttt{bos} refers to the teacher model in \texttt{Bosnian}-to-\texttt{English} translation.


At the beginning of training, multilingual LSSD also has an ``initial training stage'' for each language pair just like the bilingual LSSD, at which time the language-specific teacher doesn't work. Note that the initial training stage of different language pairs may last different epochs.
After the initial training stage, the language-specific teacher model begins working, and the student model can be guided by the teacher.
The different kinds of orange lines mean the language-specific teacher is distilling the student model and the number of working teachers is determined by the language-specific switches, which are consistent with the distillation switch of bilingual LSSD.
The blue line represents the language-specific teacher is replaced by the better-performance student from the last training epoch.
In this paper, multilingual LSSD is the superposition of multiple bilingual LSSDs and they do not affect each other.
We also summarize this process in Algorithm~\ref{alg:algorithm}. 



% Algorithm Begin=================
\begin{algorithm}[t]
\label{alg:LSSD}
\small
\caption{Language-Specific Self-Distillation} \label{alg:algorithm}
 \textbf{Input}: 
    \textit{language pairs number} $L$; 
    \textit{training sets} $\{D^{train}_l\}_{l=1}^{L}$; 
    \textit{dev sets} $\{D^{dev}_l\}_{l=1}^{L}$; 
    \textit{max training epochs} $K$; \textit{max training steps of one epoch } $T$;
    \textit{learning rate} $\eta$;\\
 \textbf{Initialize}: 
    initialize MNMT model $\theta$; for $l \in [1, L]$, set $\hat{\theta}_l=\varnothing$, $\Omega_l=off$, $\hat{\mathcal{L}}^{dev}_l=+\infty$.
\begin{algorithmic}[1] %[1] enables line numbers

\For{$k \in [1, K]$} \Comment{For each training epoch}
\For{$t \in [1, T]$} \Comment{Training stage}
\State \textit{Randomly sample a language pair} $l$. 
\State \textit{Sample a mini-batch of sentence pairs} $B^t_l$.
\If { $\Omega_l$ is on}
\State $\mathcal{L} = \mathcal{L}_{NMT}(B^t_l;\theta) + \alpha \mathcal{L}_{LSSD}(B^t_l;\theta,\hat{\theta}_l)$
\Else
\State $\mathcal{L} = \mathcal{L}_{NMT}(B^t_l;\theta)$
\EndIf
\State Update $\theta$: $\theta = \theta - \eta \cdot \nabla_{\theta}\mathcal{L}$
\EndFor

\For{$l \in [1, L]$} \Comment{Validation Stage}
\State $\mathcal{L}^{dev}_l = \mathcal{L}_{NMT}(D^{dev}_l;\theta)$
% \State $\mathcal{L}^{dev}_l=\mathcal{L}_{NMT}(D^{dev}_l;\theta), \hat{\mathcal{L}}^{dev}_l=\mathcal{L}_{NMT}(D^{dev}_l;\hat{\theta}_l)$
\If{$\mathcal{L}^{dev}_l < \hat{\mathcal{L}}^{dev}_l$}
\State $\Omega_l=off$, $\hat{\theta}_l =\theta$, $\hat{\mathcal{L}}^{dev}_l=\mathcal{L}^{dev}_l$
\Else
\State $\Omega_l=on$
\EndIf
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}
% Algorithm finished===============


% Algorithm Begin=================
% \begin{algorithm}[t]
% \small
% \caption{Language-Specific Self-Distillation algorithm} \label{alg:algorithm}
%  \textbf{Input}: 
%     \textit{language pairs number} $L$; 
%     \textit{training sets} $\{D^{train}_l\}_{l=1}^{L}$; 
%     \textit{dev sets} $\{D^{dev}_l\}_{l=1}^{L}$; 
%     \textit{max training epochs} $K$; \textit{max training steps of one epoch} $T$;
%     \textit{learning rate} $\eta$;
%     \textit{initialized model} $\theta$.\\
%  \textbf{Initialize}: 
%     \textit{For each language pair} $l \in [1, L]$\textit{, initialize language-specific best checkpoint} $\hat{\theta}_l=\theta$\textit{, index} $\hat{k}_l=1$\textit{, dev loss} $\hat{\mathcal{L}}_l^{dev} = +\infty$.
% \begin{algorithmic}[1] %[1] enables line numbers

% \For{$k \in [1, K]$} \Comment{For each training epoch}
% \For{$t \in [1, T]$} \Comment{Training stage}
% \State \textit{Randomly sample a language pair} $l$. 
% \State \textit{Sample a mini-batch of sentence pairs} $B^t_l$.
% \If {$k - \hat{k}_l > 1$ }
% \State $\mathcal{L} = \mathcal{L}_{NMT}(B^t_l;\theta) + \alpha \mathcal{L}_{LSSD}(B^t_l;\theta,\hat{\theta}_l)$
% \Else
% \State $\mathcal{L} = \mathcal{L}_{NMT}(B^t_l;\theta)$
% \EndIf
% \State Update $\theta$: $\theta = \theta - \eta \cdot \nabla_{\theta}\mathcal{L}$
% \EndFor

% \For{$l \in [1, L]$} \Comment{Validation Stage}
% \State $\mathcal{L}^{dev}_l = \mathcal{L}_{NMT}(D^{dev}_l;\theta)$
% \If{$\mathcal{L}^{dev}_l < \hat{\mathcal{L}}^{dev}_l$}
% \State $\hat{k}_l = k$, $\hat{\theta}_l =\theta$, $\hat{\mathcal{L}}^{dev}_l = \mathcal{L}^{dev}_l$
% \EndIf
% \EndFor
% \EndFor
% \end{algorithmic}
% \end{algorithm}
% Algorithm finished===============

\subsection{Formalization of LSSD} 
% The self-distillation of each language is independent, the student model can be guided by multiple teachers at the same time, and whether the teacher works in each round is determined according to the language corresponding switch. This process can be viewed as a state superposition of multiple bilingual distillations of bilingual LSSD, we do not perform distillation, but iteratively replace the teacher with the student, which has a lower loss value.
Formally, we denote the current model by $\theta$ and maintain a set of language-specific best checkpoints $\{\hat{\theta}_l\}_{l=1}^L$. In the validation stage, which is at the end of each epoch, we evaluate the performance of $\theta$ on each language pair. 
For each language pair $l$, if $\theta$ outperforms $\hat{\theta}_l$ in dev set $D^{dev}_l$, $\theta$ replaces $\hat{\theta}_l$. 
To control whether to perform teaching in the current epoch, we define a set of distillation switches $\{\Omega_l\}_{l=1}^L$. 
In the validation stage, if the current model $\theta$ exceeds the language-specific best checkpoint $\hat{\theta}_l$, we turn off the distillation switch, not performing teaching in the next epoch. 
Conversely, when the language-specific best checkpoint wins, we turn on the switch, performing teaching in the next epoch.

%The training loss of LSSD is shown in Eq.\ref{eq:total loss}.
When the language-specific distillation switch is on,
the parameters of the current model $\theta$ is updated by optimizing both 
$\mathcal{L}_\text{NMT}$ and $\alpha \cdot \mathcal{L}_\text{LSSD}$.
When the language-specific distillation switch is off, the model $\theta$ is updated only by $\mathcal{L}_\text{NMT}$, \ie{$\alpha  =0$}.
%sentence pair $(x,y)$ in the corresponding language pair $l$ and the $\theta$ mimics the output of teacher $\hat{\theta}_l$ and ground-truth labels simultaneously.
The training loss is calculated as:
\begin{align}
    \label{eq:total loss}
    \mathcal{L} &= \mathcal{L}_\text{NMT} + \alpha \mathcal{L}_\text{LSSD},
\end{align}
where the $\alpha$ is the weight of distillation loss. And $\mathcal{L}_\text{LSSD}$ is computed as the cross-entropy between the output distribution of $\hat{\theta}_l$ and $\theta$, which is formalized as:

\begin{equation}
\begin{aligned}
    \mathcal{L}_\textsc{LSSD} = -\sum\limits_{i \le |y|} \sum\limits_{w \in \mathcal{V}} &P(w|x,y_{<i};\hat{\theta}_l) \\
    &\cdot \log P(w|x,y_{<i};\theta).
\end{aligned}
\end{equation}

% \paragraph{Language-Wise Multilingual Distillation}
% When the target vocabulary contains words in diverse languages (\eg One-to-Many translation), words in non-target languages are allocated more probabilities from soft targets (\ie teacher outputs) than one-hot labels (\ie ground truth labels). This may inject some noisy into the training of MNMT models. Therefore, we only calculate distillation loss over words in the target language.


\input{tables/main_results}

\subsection{Sample-level Manipulations for LSSD} \label{subsection:IASD}
%The teacher model may also err in some translation instances. 
To prevent the potential negative transferring on some translation samples where the teacher underperforms the student, we devise three sample-level manipulations for LSSD: \textsc{LSSD-Whole}, \textsc{LSSD-Selective} and  \textsc{LSSD-Adaptive}. All of them could be generalized as rescaling the distillation loss with a sample-level weight:
\begin{align}
    \mathcal{L}_\textsc{LSSD} = \mathcal{L}_\textsc{LSSD} \times \mathcal{G},
\end{align}
where $\mathcal{G}$ is the sample-level weight which is determined by the performance difference between teacher and student. And different operations correspond different implementation of $\mathcal{G}$.

\paragraph{\textsc{LSSD-Whole}} In this manner, we equally execute distillation with the same sample-level weight on all data samples. 
In practice, it is equivalent to setting $\mathcal{G}=1$.
\textsc{LSSD-Whole} can be viewed as the base version of LSSD.

\paragraph{\textsc{LSSD-Selective}} To avert the negative impact of performing distilltaion on data samples where the teacher model errs on, we explore to only distilling samples where the teacher performs better than the student. And this is implemented as:
\begin{align}
    \mathcal{G}(x,y,\theta, \hat{\theta}_l)=\left\{
\begin{aligned}
0, &  &P(y|x;\hat{\theta}_l) < P(y|x;\theta)& \\
1, &  &P(y|x;\hat{\theta}_l) \ge P(y|x;\theta)&, \\
\end{aligned}
\right.
\end{align}
where $P(y|x;\theta)$ is the likelihood probability that model $\theta$ outputs with respect to the target sentence $y$ given the input $x$. And we compute the sentence probability by averaging probabilities over all tokens.

\paragraph{\textsc{LSSD-Adaptive}} Since a one-size-fits-all rule prohibiting distillation on a subset of samples could limit flexibility, we design \textsc{LSSD-Adaptive} changing the distillation weight according to the teacher-student performance ratio, which is implemented as:
\begin{align}
\label{eq:teacher-student performance ratio}
\mathcal{G}(x,y,\theta, \hat{\theta}_l) = min(\frac{P(y|x;\hat{\theta}_l)}{P(y|x;\theta)}, \sigma),
\end{align}
where $\sigma$ is a hyperparameter to truncate the $\mathcal{G}$ when higher than $\sigma$, value of which is set to 2 empirically\footnote{We search the optimal $\sigma$ in $\{1.0, 1,5, 2.0\}$}.


==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/4_experiments.tex <==
%====================Main results
\input{tables/results_per_languages}
% \input{tables/results_diverse}
% \input{tables/results_related}
% \input{tables/results_WMT}

\section{Experiments}

\subsection{Settings}

\paragraph{Datasets}
We conduct experiments on three datasets: the widely-used TED-8-Diverse and TED-8-Related~\citep{wang-etal-2020-balancing}, and a relative large-scale WMT dataset. 
The TED-8-Diverse contains 4 low-resource languages (\texttt{bos}, \texttt{mar}, \texttt{hin}, \texttt{mkd}) and 4 high-resource languages (\texttt{ell}, \texttt{bul}, \texttt{fra}, \texttt{kor}) to English. 
The TED-8-Related contains 4 low-resource languages (\texttt{aze}, \texttt{bel}, \texttt{glg}, \texttt{slk}) and 4 related high-resource language (\texttt{tur}, \texttt{rus}, \texttt{por}, \texttt{ces}) to English. 
Both of these two datasets have around 570K sentence pairs.
We detail the data statistics and the interpretation of language codes in Appendix~\ref{section:data statistics}.

For the WMT dataset, we consider 3 low-resource languages (\texttt{et}, \texttt{ro}, \texttt{tr}) and 3 high-resource languages (\texttt{fr}, \texttt{de}, \texttt{zh}) to English.
Totally around 5M training sentences are sampled from the parallel corpus provided by WMT14, WMT16, WMT17, and WMT18. And we use the corresponding dev and test sets for validation and evaluation. The detailed data statistics are also placed in Appendix~\ref{section:data statistics}. Compared to TED-8-Diverse and TED-8-related, the size of the WMT dataset is larger and distributed more unevenly over various languages.

For each dataset, we experiment in two multilingual translation scenarios: 1) \textsc{Many-to-One}~(M2O): translating multiple languages to English in this work; 2) \textsc{One-to-Many}~(O2M): translating English to different languages. 

%\subsection{Experimental setup}
\paragraph{Hyperparameters}
We verify the effectiveness of LSSD on the Transformer~\cite{vaswani-etal-2017-attention} as implemented in fairseq~\cite{ott-etal-2019-fairseq} with 6 layers and 8 attention heads. And we use the same hyperparameters with the previous SOTA~\citep{zhou-etal-2021-distributionally} to obtain a strong baseline. The only difference with~\citet{zhou-etal-2021-distributionally} is that we train all models for 300 epochs which is less than theirs\footnote{We also tried for more epochs, while no performance gains happened}.
For the TED-8-Diverse and TED-8-Related, we follow previous works \citet{wang-etal-2020-balancing,zhang-etal-2021-competence-based} to preprocess both datasets using sentencepiece~\citep{kudo-richardson-2018-sentencepiece} with a vocabulary size of 8\textit{K} for each language. For the WMT dataset, we preprocess data using sentencepiece with a vocabulary size of 64\textit{K} for all languages.
The complete set of hyperparameters can be found in Appendix~\ref{subsection:hyperparameters}.
All models are trained on 8 Tesla V100 GPUs.
And the performance is evaluated with BLEU score using sacreBLEU~\cite{papineni-etal-2002-bleu,post-2018-call}.
We set distillation weight $\alpha$ to 2.0 in M2O and 0.6 in O2M respectively (see section~\ref{subsection: Effect of Distillation Weight} for analysis on these choices).
% in the search the optimal distillation weight $\alpha$ for LSSD among \{0.5, 1.0, 1.5, 2.0, 2.5\} in M2O translation and among \{0.2, 0.4, 0.6, 0.8, 1.0\} in O2M translation respectively.

\paragraph{Baselines}
We compare our LSSD with: 
1) the standard-trained multilingual NMT model (\ie \textsc{Multilingual})~\citep{johnson-etal-2017-googles}; 
2) \textsc{Multi-Distill}~\citep{tan-etal-2018-multilingual}, which is also a distillation-based strategy that guides the multilingual model in each translation direction utilizing bilingual models. To re-implement \textsc{Multi-Distill}, we first train bilingual models of each language pair on all three datasets\footnote{we report performance of bilingual models in Appendix~\ref{subsection: bilingual performance}}. 
Follow previous works~\citep{tan-etal-2018-multilingual,zhang-etal-2021-competence-based}, we train bilingual models using the same model configuration and hyper-parameters with multilingual models.
For all baselines and our LSSD, the same model configuration and hyper-parameters are applied.


\begin{figure*}[th]
  \centering
    \includegraphics[clip,width=2.0\columnwidth,]{figure/diverse_baseline_with_all_modes.pdf}
    \caption{ Loss curves of the \textsc{Multilingual} baseline and LSSD in M2O (left half part) and O2M (right half part) settings on the TED-8-Diverse dataset. 
    %  The first row shows \textbf{low-resource} language pairs. The second row shows \textbf{high-resource} language pairs. The third row shows average losses. 
     The x-axis and y-axis indicate training epochs and dev losses respectively. 
    %  The solid lines are loss curves of our method. The dotted lines are loss curves of the baseline. 
     Due to space limitation, we only display 4 language pairs (2 low-resource + 2 high-resource) in each setting.}
  \label{fig:loss curve Diverse}
\end{figure*}
%============

\subsection{Main Results}
\paragraph{Overall results} 
We summarize main results into Table~\ref{tab:main results}. As we can see, 
1) on all three datasets, our LSSD significantly outperforms the baselines under M2O and O2M settings, demonstrating the effectiveness of our approach;
2) compared with previous works, LSSD achieves higher BLEU scores on the TED-8-Diverse and TED-8-Related datasets, which indicates the superiority of our method;
3) in the comparison among the three variants of LSSD, \textsc{LSSD-Adaptive} excels in M2O and \textsc{LSSD-Whole} performs best in O2M overall. To better understand this phenomenon, we analyzed the teacher-student performance ratio (detailed in Equation~\ref{eq:teacher-student performance ratio}) in M2O and O2M respectively, and discovered that this ratio varies more significantly in the challenging O2M translation than in the M2O (the variance is 0.097 in O2M and is 0.039 in M2O), which may incur an unstable training for LSSD-Adaptive.

\paragraph{Results on each language}
Looking closer at results per languages for the \textsc{Multi-Distill} and our LSSD,
we calculate the difference between \textsc{Multilingual} and \textsc{Multi-Distill} or LSSD separately in terms of BLEU, which is shown in Table~\ref{tab:results per languages}.
% For clarity, We take the mode of LSSD, which has the highest BLEU on the corresponding dataset, as the representative of LSSD respectively. 
Firstly, on all datasets and settings, \textbf{LSSD consistently outperforms the \textsc{Multilingual} baseline across all language pairs}. The improvement is up to 2.37 (\texttt{eng} $\rightarrow$\texttt{mkd}).
Secondly, Multi-Distill struggles in low-resource directions across all three datasets, which is not unexpected considering that the training data is too scarce to train trustworthy bilingual teacher models. 
However, LSSD breaks this limitation, obtaining stable improvements on \textbf{both} low-resource and high-resource language pairs, by employing multilingual NMT models that own more balanced performance as teacher models.
\input{tables/DUB_results_all}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/5_analysis.tex <==
%=============Figure: LS_loss_curve

\section{Analysis}

\subsection{Convergence Inconsistency}
\label{subsection:Convergence Inconsistency}
In this work, we propose to formalize the convergence inconsistency as the loss gap between the overall best checkpoint and language-specific best checkpoints, which is referred to as ``{\textbf{Performance Deficit}})''. 
Concretely, for each language pair $l$, we accumulate the dev loss differences between the overall best checkpoint $\theta$ and the corresponding language-specific best checkpoint $\hat{\theta}_l$.
We give a formal definition as:
\begin{align}
    \text{DUB}(\theta, \{\hat{\theta_l}\}^L_{l=1}) \!=\! \sum_{l=1}^{L} (\mathcal{L}(\theta, D_l^{dev})
    \!-\! \mathcal{L}(\hat{\theta}_l, D_l^{dev})).
\end{align}
% 下面这句话，如果没篇幅可以考虑删除
Note that the performance deficit is a non-negative value because $\mathcal{L}(\theta, D_l^{dev})$ is always greater than or equal to $\mathcal{L}(\hat{\theta}_l, D_l^{dev})$.
We list the performance deficit of the \textsc{Multilingual} baseline and our LSSD in Table~\ref{tab:distance to upper bound of all method in all datsets and settings.}. 
As observed, the performance deficit of LSSD is significantly lower than the baseline (decreased 57\% on average), which proves the efficacy of LSSD in remedying convergence inconsistency.


\subsection{Multiple Teachers vs. Single Teacher}
\input{tables/single_teacher_results}
To provide light on the necessity of using language-specific best checkpoints as teacher models, we conduct ablation study in Table~\ref{tab:multiple teachers vs. single teacher.}. The STSD (Single Teacher Self-Distillation) uses the overall best checkpoint instead of language-specific best checkpoints to guide the training of multilingual NMT models. 
To make a fair comparison, we report the results of \textsc{LSSD-Whole}.
% As indicated, STSD reaches a 20\%\textasciitilde60\% improvement compared to the improvement of LSSD in the M2O translation. 
As indicated, the gains from STSD over the baseline only account for 20\% to 60\% of LSSD's gains in the M2O translation.
Even more, STSD fails to enhance the O2M translation. 
These results show that the multilingual model gains a great deal from tailored language-specific teachers indeed.

\subsection{Comparison of Loss Curves}
\label{subsection:Effectiveness on Alleviating Over-fitting}
To better comprehend how each approach affects the model training process, we analyze different methods from the perspective of loss curves, as illustrated in Figure~\ref{fig:loss curve Diverse}. 
Firstly, comparing the loss curves of the \textsc{Multilingual} baseline with LSSD (solid lines vs. dotted lines), it is clear that the baseline suffers from serious over-fitting in low-resources (\eg{\texttt{bos} $\leftrightarrow$ \texttt{eng}}). By letting the model \textit{recall} previous checkpoints, LSSD mitigates the over-fitting, which delays the convergence to lengthen the training time for high-resource languages.
Secondly, comparing the loss curves of baselines in M2O and O2M (dotted lines in left vs. right half section), it is observed that M2O suffers from more serious over-fitting than O2M. 
This explains why M2O benefits more from LSSD than O2M.
Lastly, contrasting the three modes of \textsc{LSSD}, \textsc{LSSD-Adaptive} performs better in M2O and achieves comparable with \textsc{LSSD-Whole} in O2M in terms of dev loss.
% Complete loss curves on both datasets and settings could be found in Appendix B.

\subsection{Effect of Distillation Weight $\alpha$}
\label{subsection: Effect of Distillation Weight}
As Equation~\ref{eq:total loss} shows, LSSD trains multilingual NMT models with NMT loss and the $\alpha$-weighted distillation loss jointly. We demonstrate the effect of different $\alpha$ on LSSD in Figure~\ref{fig:Effect on weight}. 
As we can see, the optimal weight for O2M ($\alpha=0.6$) is smaller than which for M2O ($\alpha=2.0$).
We conjecture this is due to the fact that O2M converges later than M2O (see Section~\ref{subsection:Effectiveness on Alleviating Over-fitting}), meaning that O2M models might learn from immature teachers for more epochs. Consequently, a lower distillation strength is more suited to eliminating this danger.

\begin{figure}[t]
  \centering
    \includegraphics[clip,width=1.0\columnwidth,]{figure/Effect_on_weight_Diverse.pdf}
    \caption{Effect of different distillation weights on LSSD. For clarity, we take \textsc{LSSD-Whole} as the representative of LSSD.}
  \label{fig:Effect on weight}
\end{figure}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/6_related_works.tex <==
\section{Related Works}
\subsection{Advances in Multilingual NMT}
% Multilingual neural machine translation has attracted much attention in recent years~\citep{dong-etal-2015-multi,johnson-etal-2017-googles,arivazhagan2019massively,fan2020beyond}.
% And \newcite{10.1145/3406095} have made a comprehensively review for MNMT works until 2019.
Recently, multilingual NMT mainly focuses on: 1) designing effective parameters sharing strategy \cite{zhang-etal-2021-share,zhu-etal-2021-counter-interference,xie-etal-2021-importance,lin-etal-2021-learning}; 2) obtaining language-agnostic representations ~\cite{zhu-etal-2020-language,pan-etal-2021-contrastive}; 3) incorporating pre-training models ~\cite{siddhant-etal-2020-leveraging,wang-etal-2020-multi}; 4) resolving the data imbalance among diverse languages~\cite{wang-etal-2020-balancing,wu-etal-2021-uncertainty,zhang-etal-2021-competence-based,zhou-etal-2021-distributionally}.
    % \paragraph{Parameters sharing} To minimum the negative transferring (i.e., parameters interference) among languages, \newcite{zhang2021share} add a language-specific sub-layer for each language to choose between with the shared Feed-forward sub-layer. Similarly, \newcite{zhu-etal-2021-counter-interference} add adapters to cooperate with the shared network. Both of \newcite{xie-etal-2021-importance} and \newcite{lin-etal-2021-learning} propose to learn a language-specific sub-network for each language with neuron pruning.
    % \paragraph{Universal representation} To maximum the positive transferring, \newcite{zhu-etal-2020-language} insert a interlingua module to obtain language-agnostic representations. \newcite{pan-etal-2021-contrastive} close the gap among representations of different languages with contrastive learning. \newcite{lin-etal-2020-pre} train a MNMT model in the aligned code-switched parallel data.
    % \paragraph{Pre-training} To make use of monolingual data, \newcite{siddhant-etal-2020-leveraging} pre-train the MNMT model on monolingual data with MASS~\cite{song2019mass} training objective. \newcite{wang-etal-2020-multi} pre-train the model with MLM~\cite{devlin-etal-2019-bert} and DAE~\cite{lewis-etal-2020-bart} training objectives. \newcite{tang2020multilingual} train an mBART-initialized MNMT model. \newcite{sun-etal-2021-multilingual-translation} explore to combine mBERT~\cite{devlin-etal-2019-bert} and GPT~\cite{radford2018improving} into a MNMT model.
    % \paragraph{Balancing Training} To resolve the data imbalance in MNMT, it is proposed to dynamically adjust the sampling strategy with gradient similarities~\cite{wang-etal-2020-balancing}, uncertainty~\cite{wu-etal-2021-uncertainty}. \newcite{zhang-etal-2021-competence-based} propose to learn a MNMT in a curriculum learning manner. And \newcite{zhou-etal-2021-distributionally} train the model with ditributionally robustness optimization.
Different from them, LSSD is designed for alleviating the convergence inconsistency, which is ignored by existing works.

   



\subsection{Knowledge Distillation in NMT}
To the best of our knowledge, \newcite{kim-rush-2016-sequence} first apply knowledge distillation in bilingual NMT and propose a sequence-level distillation.
\newcite{wei-etal-2019-online} propose to avoid over-fitting by guiding the training process with best checkpoints. 

In multilingual NMT, \newcite{tan-etal-2018-multilingual} use knowledge distillation to close the gap between the multilingual NMT model and bilingual models. 
However, their work is based on the hypothesis that there are sufficient training data for each language pair to prepare a promising bilingual teacher. 
In fact, most languages face the resource-scarcity problem. 
In our work, LSSD's teacher is the multilingual model, which has a better performance for low resource language translation via transfer learning.
And we further develop three sample-level operations for LSSD via weighing teacher and student performance.


==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/7_conclusion.tex <==
\section{Conclusion}
In this work, we propose a novel training strategy \textbf{L}anguage-\textbf{S}pecific \textbf{S}elf-\textbf{D}istillation (LSSD) to remedy the convergence inconsistency in multilingual neural machine translation. Moreover, we devise three sample-level manipulations for LSSD. 
Experimental results on three datasets demonstrate that LSSD achieves SOTA performance. 
Through analysis experiments, we also find that: 1) LSSD significantly mitigates the convergence inconsistency (decreased 57\% on average), which is quantified by performance deficit;
2) both low-resource and high-resource languages benefit from LSSD.
% 3) \textsc{Many-to-One} converges earlier than \textsc{One-to-Many}
% In the future, we will explore the effectiveness of  our method in multi-task learning.
% In the future, we will apply our method to larger datasets and massive language pairs to study the upper-bound of our method.

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/8_limitations.tex <==
\section{Limitations}
Same with other distillation-based works~\citep{hinton2015distilling,tan-etal-2018-multilingual}, LSSD takes some extra training overhead. Taking the training in TED-8-Diverse M2O as an example, the \textsc{Baseline} and \textsc{LSSD-Whole} spend 5.7 hours and 7.6 hours respectively. 
However, it is worth noting that our method doesn't affect the inference speed of the model.
% \textsc{LSSD-Selective} and \textsc{LSSD-Adaptive} spend 8 hours as performing more operations. 
% In terms of GPU memory usage, LSSD takes up about extra 2.4GB of memory mainly for storing teacher models (each one takes about 300MB).


==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/DUB_results.tex <==
\begin{table}[t]
\small
\renewcommand\tabcolsep{2.0pt}
\centering
\begin{tabular}{l|cc|cc|cc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textsc{Diverse}} & \multicolumn{2}{c|}{\textsc{Related}} & \multicolumn{2}{c}{\textsc{WMT}} \\
& \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} \\
\midrule

\textsc{Multilingual} & 0.27 & 0.64 & 0.57 & 0.51 & 0.75 & 1.09\\

LSSD & 0.21 & 0.15 & 0.32 & 0.30 & 0.25 & 0.32 \\

$\Delta$ & $\downarrow$22\% & $\downarrow$77\% & $\downarrow$44\% & $\downarrow$41\% & $\downarrow$67\% & $\downarrow$71\% \\
\bottomrule
\end{tabular}
\caption{\textbf{DUB} (Distance to Upper-Bound) of the baselines and LSSD on all datasets.}
\label{tab:distance to upper bound in all datsets and settings.}
\end{table}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/DUB_results_all.tex <==
\begin{table}[t]
\small
\renewcommand\tabcolsep{2.0pt}
\centering
\begin{tabular}{l|cc|cc|cc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textsc{\textbf{Diverse}}} & \multicolumn{2}{c|}{\textsc{\textbf{Related}}} & \multicolumn{2}{c}{\textsc{\textbf{WMT}}} \\
& M2O & O2M & M2O & O2M & M2O & O2M \\
\midrule

\textsc{Multilingual} & 0.27 & 0.64 & 0.57 & 0.51 & 0.75 & 1.09\\

\textsc{LSSD-Whole} & 0.21 & \textbf{0.15} & 0.32 & 0.30 & 0.25 & \textbf{0.32} \\

\textsc{LSSD-Selective} & 0.24 & 0.37 & 0.35 & 0.29 & 0.21 & 0.36 \\

\textsc{LSSD-Adaptive} & \textbf{0.19} & 0.35 & \textbf{0.16} & \textbf{0.26} & \textbf{0.14} & 0.44 \\

\bottomrule
\end{tabular}
\caption{Performance deficit of the \textsc{Multilingual} baseline and our LSSD. Bold indicates the lowest value under each setting. Compared to the baseline, LSSD reduces this deficit by 57\% on average.}
\label{tab:distance to upper bound of all method in all datsets and settings.}
\end{table}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/bilingual_results_WMT.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccc | c}
    \toprule
        & \textbf{Method} & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr}	& \textbf{Avg.} \\
    \midrule
        \multirow{2}{*}{M2O} 
        & \textsc{Bilingual} & 0.78 & 5.00 & 5.99 & 11.60 & \textbf{27.94} & \textbf{33.57} & 14.15 \\
        & \textsc{Multilingual} & \textbf{9.89} & \textbf{23.12} & \textbf{16.92} & \textbf{12.72} & 26.68 & 31.57 & \textbf{20.15}\\
        \midrule
        
        
        \multirow{2}{*}{O2M} 
        & \textsc{Bilingual} & 0.34 & 3.34 & 4.76 & 19.38 & \textbf{24.11} & \textbf{36.07} & 14.67  \\
        & \textsc{Multilingual} & \textbf{8.83} & \textbf{18.42} &\textbf{ 13.34} & \textbf{20.78} & 21.11 & 31.93 & \textbf{19.07}  \\
        
    \bottomrule
    \end{tabular}
    \caption{BLEU scores of bilingual models and the multilingual model on the WMT dataset.
    Languages are ordered increasingly by data size from left to right.
    Bold indicates the better performance. We can see that the \textsc{Bilingual} model far outperforms the \textsc{Multilingual} on the high-source \texttt{fr}$\leftrightarrow$\texttt{en} and \texttt{de}$\leftrightarrow$\texttt{en}.
    However, when the training data is limited, the \textsc{Bilingual} model lags far behind the \textsc{Multilingual}.
    }
    \label{tab:bilingual results wmt}
    \vspace{-3mm}
\end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/bilingual_results_diverse.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccccc |c}
    \toprule
        & \textbf{Method} & \textbf{bos} & \textbf{mar} & \textbf{hin} & \textbf{mkd} & \textbf{ell} & \textbf{bul} & \textbf{fra}   & \textbf{kor} & \textbf{Avg.} \\
    \midrule
        \multirow{2}{*}{M2O} 
        & \textsc{Bilingual} & 5.64 & 3.35 & 9.90 & 19.66 & 37.00 & 38.85 & \textbf{40.67} & \textbf{19.25} & 21.79 \\
        & \textsc{Multilingual} & \textbf{25.78} & \textbf{11.25} & \textbf{24.30} & \textbf{33.38} & \textbf{38.40} & \textbf{39.34} & 40.43 & 19.15 & \textbf{29.00} \\
        
        \midrule
        
        \multirow{2}{*}{O2M} 
        & \textsc{Bilingual} & 3.89 & 2.47 & 8.16 & 13.98 & 30.97 & 34.21 & 38.53 & 7.70 & 17.49 \\
        & \textsc{Multilingual} & \textbf{17.04} & \textbf{4.96} & \textbf{15.99} & \textbf{25.34} & \textbf{33.27} & \textbf{36.31} & \textbf{40.81} & \textbf{9.08} & \textbf{22.85} \\
    \bottomrule
    \end{tabular}
    \caption{BLEU scores of bilingual models and the multilingual model on the TED-8-Diverse dataset.
    Languages are ordered increasingly by data size from left to right. Bold indicates the higher BLEU score. We can find that the \textsc{Multilingual} model consistently outperforms the \textsc{Bilingual} model on each language pair except for \texttt{fra}$\rightarrow$\texttt{eng} and \texttt{kor}$\rightarrow$\texttt{eng}.}
    \label{tab:bilingual results diverse}
    \vspace{-3mm}
\end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/bilingual_results_related.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccccc | c}
    \toprule
        & \textbf{Method} & \textbf{aze} & \textbf{bel}	& \textbf{glg} & \textbf{slk} & \textbf{tur} & \textbf{rus} & \textbf{por} & \textbf{ces}	& \textbf{Avg.}\\
    \midrule
        \multirow{2}{*}{M2O} 
        & \textsc{Bilingual} & 2.16 & 1.8 & 10.1 & 23.62 & 26.51 & 24.97 & 44.53 & 25.77 & 19.93 \\
        & \textsc{Multilingual} & \textbf{13.11} & \textbf{19.57} & \textbf{30.14} & \textbf{32.36} & \textbf{27.07} & \textbf{25.85} & \textbf{44.89} & \textbf{29.66} & \textbf{27.83}\\
        \midrule
        
        
        \multirow{2}{*}{O2M} 
        & \textsc{Bilingual} & 1.59 & 1.78 & 9.25 & 17.62 & 14.51 & 19.59 & 39.15 & 17.97 & 15.18 \\
        & \textsc{Multilingual} &\textbf{7.40} & \textbf{13.09} & \textbf{25.71} & \textbf{25.66} & \textbf{16.93} & \textbf{20.94} & \textbf{41.68} & \textbf{23.35} & \textbf{21.85} \\
        
    \bottomrule
    \end{tabular}
    \caption{BLEU scores of bilingual models and the multilingual model on the TED-8-related dataset.
    Languages are ordered increasingly by data size from left to right.
    Bold indicates the higher BLEU score.
    We can find that the \textsc{Multilingual} model consistently outperforms the \textsc{Bilingual} model on all language pairs.}
    \label{tab:bilingual results related}
    \vspace{-3mm}
\end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/data_statistics_TED.tex <==
\begin{table}[th]
\small
\renewcommand\tabcolsep{3.0pt}
\centering

\begin{tabular}{lc|lc}
\toprule
\multicolumn{2}{c|}{\textsc{Diverse}} & \multicolumn{2}{c}{\textsc{Related}}  \\
language & \#num & language & \#num \\
% & \textbf{Related} & \textbf{Diverse} & \textbf{Related} & \textbf{Diverse} \\
\midrule
\texttt{bos} (Bosnian) & 5,664 & 
\texttt{bel} (Belarusian) & 4,509 \\

\texttt{mar} (Marathi) & 9,840 & 
\texttt{aze} (Azerbaijani) & 5,946 \\

\texttt{hin} (Hindi) & 18,798 & 
\texttt{glg} (Glacian) & 10,017 \\

\texttt{mkd} (Macedonian) & 25,335 & 
\texttt{slk} (Slovak) & 61,470 \\

\texttt{ell} (Greek) & 134,327 & 
\texttt{cse} (Czech) & 103,093 \\

\texttt{bul} (Bulgarian) & 174,444 & 
\texttt{tur} (Turkish) & 182,470 \\

\texttt{fra} (French) & 192,304 & 
\texttt{por} (Portuguese) & 184,755 \\

\texttt{kor} (Korean) & 205,640 & 
\texttt{rus} (Russian) & 208,458 \\
\bottomrule
\end{tabular}
\caption{Data statistics for the TED-8-Diverse dataset and the TED-8-Related dataset. `\#num' refers to the number of sentence pairs in the training set.}
\label{tab:data statistics.}
\end{table}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/data_statistics_WMT.tex <==
\begin{table}[th]
\small
\renewcommand\tabcolsep{3.0pt}
\centering

\begin{tabular}{l|ccc}
\toprule
Language & Data Source & \#num \\
\midrule

\texttt{tr} (Turkish) & WMT17 & 5,000 \\

\texttt{ro} (Romanian) & WMT16 & 10,000 \\

\texttt{et} (Estonian) & WMT18 & 80,000 \\

\texttt{zh} (Chinese) & WMT17 & 400,000 \\

\texttt{de} (German) & WMT14 & 1,500,000 \\

\texttt{fr} (French) & WMT14 & 3,000,000 \\

\bottomrule
\end{tabular}
\caption{Data statistics for the WMT dataset. `\#num' refers to the number of sentence pairs in the training set.}
\label{tab:data statistics WMT.}
\end{table}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/main_results.tex <==
\begin{table*}[!t]
\small
% \renewcommand\tabcolsep{2.0pt}
\centering
\begin{tabular}{l|cc|cc|cc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{\textsc{Diverse}}} & \multicolumn{2}{c|}{\textbf{\textsc{Related}}} & \multicolumn{2}{c}{\textbf{\textsc{WMT}}} \\
& \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} \\

\midrule
\midrule
\multicolumn{7}{c}{\textit{Baselines}} \\
\midrule

\textsc{Multilingual} & 29.00 & 22.85 & 27.83 & 21.85 & 20.15 & 19.07\\
\textsc{Multi-Distill}~\cite{tan-etal-2018-multilingual} &  29.52 & 22.31 & 26.60 & 21.70 & 20.18 & 18.57 \\

\midrule
\midrule
\multicolumn{7}{c}{\textit{Previous Works}} \\
\midrule

MultiDDS-S~\cite{wang-etal-2020-balancing}$^*$
& 27.00 & 18.24 & 25.52 & 17.32 & -- & -- \\
MultiUAT~\cite{wu-etal-2021-uncertainty}$^*$
& 27.83 & 19.76 & 26.39 & 18.64 & -- & -- \\
CCL-M~\cite{zhang-etal-2021-competence-based}$^*$
& 28.34 & 19.53 & 26.73 & 18.89 & -- & -- \\
$\chi$-IBR~\cite{zhou-etal-2021-distributionally}$^*$
& 29.74 & 23.44 & 28.71 & 22.21 & -- & -- \\



\midrule
\midrule
\multicolumn{7}{c}{\textit{Our Proposed Approaches}} \\
\midrule

LSSD-Whole  & 30.57$^\dagger$ & \textbf{23.55}$^\dagger$ & 29.28$^\dagger$ & 22.20$^\dagger$ & 21.05$^\dagger$ & \textbf{19.76}$^\dagger$\\
LSSD-Selective & 30.24$^\dagger$ & 23.16 & 28.65$^\dagger$ & 22.15$^\dagger$ & \textbf{21.17}$^\dagger$ & 19.32$^\dagger$ \\
LSSD-Adaptive & \textbf{30.77}$^\dagger$ & 23.39 & \textbf{29.40}$^\dagger$ & \textbf{22.27}$^\dagger$ & 20.96$^\dagger$ & 19.48$^\dagger$\\
\bottomrule
\end{tabular}
\caption{BLEU scores on TED-8-Diverse (\textsc{Diverse}) and TED-8-Related (\textsc{Related}) and WMT datasets.
%  The up section shows results of previous works. The middle section shows results of two baselines implemented by us. The bottom section shows results of our LSSD. 
Bold indicates the highest BLEU value on each setting. 
`*' represents results taken from original papers.
 ``M2O'' means Many-to-One translation. ``O2M'' means One-to-Many translation. 
 `$\dagger$' means significantly better than \textsc{Multilingual} with t-test $p<0.01$.}
\label{tab:main results}
\end{table*}
%====================Main results Finished


% \begin{table*}[!t]
% \small
% % \renewcommand\tabcolsep{2.0pt}
% \centering
% \begin{tabular}{l|cc|cc}

% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{\textsc{Diverse}}} & \multicolumn{2}{c}{\textbf{\textsc{Related}}} \\
% & \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} \\
% \midrule
% \multicolumn{5}{c}{\textbf{Previous Works}} \\
% \midrule
% MultiDDS-S~\cite{wang-etal-2020-balancing}$^*$
% & 27.00 & 18.24 & 25.52 & 17.32 \\
% MultiUAT~\cite{wu-etal-2021-uncertainty}$^*$
% & 27.83 & 19.76 & 26.39 & 18.64 \\
% CCL-M~\cite{zhang-etal-2021-competence-based}$^*$
% & 28.34 & 19.53 & 26.73 & 18.89 \\
% $\chi$-IBR~\cite{zhou-etal-2021-distributionally}$^*$
% & 29.74 & 23.44 & 28.71 & 22.21 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Baselines}} \\
% \midrule
% \textsc{Multilingual} & 29.00 & 22.85 & 27.83 & 21.85 \\
% \textsc{Multi-Distill}~\cite{tan2018multilingual} &  29.52 & 22.31 & 26.60 & 18.75 \\
% \midrule
% \multicolumn{5}{c}{\textbf{Ours}} \\
% \midrule
% LSSD-Whole  & 30.57 & \textbf{23.55} & 29.28 & 22.20 \\
% LSSD-Selective & 30.24 & 23.16 & 28.65 & 22.15 \\
% LSSD-Adaptive & \textbf{30.77} & 23.39 & \textbf{29.40} & \textbf{22.27} \\
% \bottomrule
% \end{tabular}
% \caption{BLEU scores on TED-8-Diverse (\textsc{Diverse}) and TED-8-Related (\textsc{Related}) datasets.
% %  The up section shows results of previous works. The middle section shows results of two baselines implemented by us. The bottom section shows results of our LSSD. 
% The highest BLEU value on each setting is in bold. 
% `*' represents results taken from original papers.
%  ``M2O'' means Many-to-One translation. ``O2M'' means One-to-Many translation.}
% \label{tab:main results}
% \end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/results_WMT.tex <==

\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccc |c}
    \toprule
        & \textbf{Method} & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr} & \textbf{Avg.} \\
    \midrule
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -0.84 & -1.40 & +0.10 & +0.78 & \textbf{+0.71} & \textbf+0.82 & +0.03 \\
        
        & LSSD & \textbf{+0.64} & \textbf{+1.25} & \textbf{+1.58} & \textbf{+0.8} & +0.7 & \textbf{+1.1} & \textbf{+1.02} \\
        \midrule
        
        \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -2.42 & -2.26 & -0.69 & +0.58 & \textbf{+0.87} & \textbf{+0.92}  & -0.50 \\
        
        & LSSD & \textbf{+0.81} & \textbf{+0.53} & \textbf{+0.48} & \textbf{+1.0} & +0.68 & +0.66 & \textbf{+0.69} \\
    \bottomrule
    \end{tabular}
    \caption{BLEU scores improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline on the \textbf{WMT} dataset.
    We take the \textsc{LSSD-Selective} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold values indicate the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:WMT results}
    \vspace{-3mm}
\end{table*}

% \begin{table*}[th]
% \renewcommand\tabcolsep{3.5pt} 
% \small
%     \centering
%     \begin{tabular}{l | ccccccc | ccccccc}
%     \toprule
%         \multirow{2}{*}{Method} & \multicolumn{7}{c|}{\textbf{\textsc{Many-to-One}}} & \multicolumn{7}{c}{\textbf{\textsc{One-to-Many}}} \\ 
%         & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr} & \textbf{Avg.} 
%         & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr} & \textbf{Avg.} \\
%         \midrule
        
%         \textsc{Multilingual} & 9.89 & 23.12 & 16.92 & 12.72 & 26.68 & 31.57 & 20.15 
%         & 8.83 & 18.42 & 13.34 & 20.78 & 21.11 & 31.93 & 19.07 \\
        
%         \textsc{Multi-Distill} & 9.05 & 21.72 & 17.02 & 13.50 & \textbf{27.39} & 32.39 & 20.18 
%         & 6.41 & 16.16 & 12.65 & 21.36 & \textbf{21.98} & 32.85 & 18.57 \\
%         \midrule
        
%         \textsc{LSSD-Whole} & \textbf{10.62} &\textbf{ 24.76} & 18.37 & 12.99 & 27.26 & 32.32 & 21.05 
%         & 9.47 & \textbf{18.85} & \textbf{13.85} & \textbf{21.38} & 21.87 & \textbf{32.98} & \textbf{19.73} \\
        
%         \textsc{LSSD-Select} & 10.53 & 24.37 & \textbf{18.50} & \textbf{13.52} & 27.38 & \textbf{32.67} & \textbf{21.17} 
%         & 9.05 & 18.44 & 13.52 & 20.98 & 21.58 & 32.32 & 19.32 \\
        
%         \textsc{LSSD-Adapt} & 10.39 & 24.63 & 18.18 & 13.19 & 27.01 & 32.08 & 20.91 
%         & \textbf{9.51} & 18.73 & 13.47 & 21.16 & 21.45 & 32.56 & 19.48 \\
%     \bottomrule
%     \end{tabular}
%     \caption{BLEU scores of two baselines and our LSSD on the WMT dataset. 
%     Languages are ordered increasingly by data size from left to right. 
%     \textbf{Bold} indicates the highest value.}
%     \label{tab:WMT results}
%     \vspace{-3mm}
% \end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/results_diverse.tex <==
%====================Diverse results
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccccc |c}
    \toprule
        & \textbf{Method} & \textbf{bos} & \textbf{mar} & \textbf{hin} & \textbf{mkd} & \textbf{ell} & \textbf{bul} & \textbf{fra}   & \textbf{kor} & \textbf{Avg.} \\
    \midrule
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -0.76 & -0.39 & -0.86 & +0.58 & +1.65 & +1.23 & +1.30 & +1.36 & +0.52 \\
        
        & LSSD & \textbf{+1.98} & \textbf{+1.00} & \textbf{+1.30} & \textbf{+2.17} & \textbf{+2.24} & \textbf{+1.81} & \textbf{+1.54} & \textbf{+2.10} & \textbf{+1.77} \\
        \midrule
        
        \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -3.44 & -0.87 & -1.26 & +0.41 & +0.49 & +0.35 & \textbf{+0.06} & -0.04  & -0.54 \\
        
        & LSSD & \textbf{+0.93} & \textbf{+0.37} & \textbf{+0.52} & \textbf{+2.37} & \textbf{+0.75} & \textbf{+0.39} & +0.04 & \textbf{+0.20} & \textbf{+0.70} \\
    \bottomrule
    \end{tabular}
    \caption{BLEU scores improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline on the \textbf{TED-8-Diverse} dataset.
    We take the \textsc{LSSD-Adaptive} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold values indicate the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:diverse results}
    \vspace{-3mm}
\end{table*}
%====================Diverse results Finished

% old version
% \begin{table*}[t]
% \small
%     \centering
%     \begin{tabular}{l|l | cccccccc |c}
%     \toprule
%         & \textbf{Method} & \textbf{bos} & \textbf{mar} & \textbf{hin} & \textbf{mkd} & \textbf{ell} & \textbf{bul} & \textbf{fra}   & \textbf{kor} & \textbf{Avg.} \\
%     \midrule
%         \multirow{3}{*}{M2O} & \textsc{Baseline} & 25.78 & 11.25 & 24.30 & 33.38 & 38.40 & 39.34 & 40.43 & 19.15  &  29.00\\
%         & LSSD & \textbf{27.33} & \textbf{12.34} & \textbf{24.87} & \textbf{35.37} & \textbf{40.12} & \textbf{41.41} & \textbf{42.04} & \textbf{21.24} & \textbf{30.59}\\
%         & $\Delta$ & +1.55 & +1.09 & +0.57 & +1.99 & +1.72 & +2.07 & +1.61 & +2.09 & +1.59 \\
%         \midrule
        
%         \multirow{3}{*}{O2M} & \textsc{Baseline} & 17.04 & 4.96 & 15.99 & 25.34 & 33.27 & 36.31 & 40.81 & 9.08  & 22.85 \\
%         & LSSD & \textbf{17.97} & \textbf{5.33} & \textbf{16.51} & \textbf{27.71} & \textbf{34.02} & \textbf{36.70} & \textbf{40.85} & \textbf{9.28} & \textbf{23.55} \\
%         & $\Delta$ & +0.93 & +0.37 & +0.52 & +2.37 & +0.75 & +0.39 & +0.04 & +0.20 & +0.70\\
%     \bottomrule
%     \end{tabular}
%     \caption{BLEU scores of the baseline and LSSD on the test set of TED-8-Diverse dataset. Bold values indicate the best performance for each language pair. Languages are ordered increasingly by data size from left to right.}
%     \label{tab:diverse results}
%     \vspace{-3mm}
% \end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/results_per_languages.tex <==
%====================Diverse results
\begin{table*}[t]
\renewcommand\tabcolsep{4.0pt}
\small
    \centering
    \begin{tabular}{c | c | c | cccccccc |c}
    \toprule
        % Diverse
        \textbf{Dataset} & \textbf{Setting} & \textbf{Method} & \textbf{bos} & \textbf{mar} & \textbf{hin} & \textbf{mkd} & \textbf{ell} & \textbf{bul} & \textbf{fra}   & \textbf{kor} & \textbf{Avg.} \\
    \midrule
        % M2O
        \multirow{4}{*}{\rotatebox{90}{\textsc{Diverse\ \ }}} &
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -0.76 & -0.39 & -0.86 & +0.58 & +1.65 & +1.23 & +1.30 & +1.36 & +0.52 \\
        & & LSSD & \textbf{+1.98} & \textbf{+1.00} & \textbf{+1.30} & \textbf{+2.17} & \textbf{+2.24} & \textbf{+1.81} & \textbf{+1.54} & \textbf{+2.10} & \textbf{+1.77} \\
    % \midrule
        \cmidrule{2-12}
        % \cmidrule{2-2} \cmidrule{3-3} \cmidrule{4-11} \cmidrule{12-12}
        %O2M
        & \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -3.44 & -0.87 & -1.26 & +0.41 & +0.49 & +0.35 & \textbf{+0.06} & -0.04  & -0.54 \\
        & & LSSD & \textbf{+0.93} & \textbf{+0.37} & \textbf{+0.52} & \textbf{+2.37} & \textbf{+0.75} & \textbf{+0.39} & +0.04 & \textbf{+0.20} & \textbf{+0.70} \\
    \midrule
    \midrule
    
        % Related
        & & & \textbf{aze} & \textbf{bel}	& \textbf{glg} & \textbf{slk} & \textbf{tur} & \textbf{rus} & \textbf{por} & \textbf{ces}	& \textbf{Avg.}\\
    \midrule
        % M2O
        \multirow{4}{*}{\rotatebox{90}{\textsc{Related\ \ }}} &
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -4.31 & -6.38 & -4.87 & +0.09 & \textbf{+1.52} & \textbf{+1.16} & \textbf{+1.62} & +1.33 & -1.23 \\
        & & LSSD & \textbf{+1.53} & \textbf{+2.35} & \textbf{+1.70} & \textbf{+1.47} & +1.18 & +1.04 & +1.43 & \textbf{+1.82} & \textbf{+1.57}\\
        % \midrule
        \cmidrule{2-12}
        % O2M
        & \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -0.32 & -0.64 & +0.14 & +0.27 & -0.20 & -0.17 & +0.09 & -0.31 & -0.15 \\
        & & LSSD & \textbf{+0.15} & \textbf{+0.12} & \textbf{+0.50} & \textbf{+0.32} & \textbf{+0.68} & \textbf{+0.20} & \textbf{+0.54} & \textbf{+0.32} & \textbf{+0.35} \\
    \midrule
    \midrule
    
        % WMT
        & & & \textbf{tr} & \textbf{ro} & \textbf{et} & \textbf{zh} & \textbf{de} & \textbf{fr} & -- & -- & \textbf{Avg.} \\
    \midrule
        % M2O
        \multirow{4}{*}{\rotatebox{90}{\textsc{WMT\ \ }}} & \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -0.84 & -1.40 & +0.10 & \textbf{+0.78} & \textbf{+0.71} & \textbf{+0.82} & -- & -- & +0.03 \\
        & & LSSD & \textbf{+0.79} & \textbf{+1.3} & \textbf{+1.29} & +0.32 & +0.5 & +0.68 & -- & -- & \textbf{+0.81} \\
        % \midrule
        \cmidrule{2-12}
        % O2M
        & \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -2.42 & -2.26 & -0.69 & +0.58 & \textbf{+0.87} & \textbf{+0.92} & -- & -- & -0.50 \\
        & & LSSD & \textbf{+0.81} & \textbf{+0.53} & \textbf{+0.48} & \textbf{+1.00} & +0.68 & +0.66& -- & -- & \textbf{+0.69} \\
    \bottomrule
    \end{tabular}
    \caption{BLEU score improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline.
    For clarity, we take \textsc{LSSD-Adaptive} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold indicates the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:results per languages}
    \vspace{-3mm}
\end{table*}

% On the TED-8-Diverse and TED-8-Related datasets, We take \textsc{LSSD-Adaptive} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively. On the WMT dataset, we take \textsc{LSSD-Selective} and \textsc{LSSD-Whole} as the representatives in M2O and O2M translation for their superiority.

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/results_related.tex <==
%====================Related results
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccccc | c}
    \toprule
        & \textbf{Method} & \textbf{aze} & \textbf{bel}	& \textbf{glg} & \textbf{slk} & \textbf{tur} & \textbf{rus} & \textbf{por} & \textbf{ces}	& \textbf{Avg.}\\
    \midrule
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -4.31 & -6.38 & -4.87 & +0.09 & \textbf{+1.52} & \textbf{+1.16} & \textbf{+1.62} & +1.33 & -1.23 \\
        & LSSD & \textbf{+1.53} & \textbf{+2.35} & \textbf{+1.7} & \textbf{+1.47} & +1.18 & +1.04 & +1.43 & \textbf{+1.82} & \textbf{+1.57}\\
        \midrule
        
        
        \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -5.57 & -10.89 & -5.54 & -1.10 & -0.54 & +0.33 & -0.26 & -1.17 & -3.10 \\
        & LSSD & \textbf{+0.37} & \textbf{+0.77} & \textbf{+0.69} & \textbf{+0.48} & \textbf{+0.36} & \textbf{+0.43} & \textbf{+0.04} & \textbf{+0.23} & \textbf{+0.42} \\
        
    \bottomrule
    \end{tabular}
    \caption{BLEU scores improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline on the \textbf{TED-8-Related} dataset. 
    We take the \textsc{LSSD-Adaptive} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold values indicate the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:related results}
    \vspace{-3mm}
\end{table*}
%====================Related results Finished

% old version
% \begin{table*}[t]
% \small
%     \centering
%     \begin{tabular}{l|l | cccccccc | c}
%     \toprule
%         & \textbf{Method} & \textbf{aze} & \textbf{bel}	& \textbf{glg} & \textbf{slk} & \textbf{tur} & \textbf{rus} & \textbf{por} & \textbf{ces}	& \textbf{Avg.}\\
%     \midrule
%         \multirow{3}{*}{M2O} & \textsc{Baseline} & 13.11 & 19.57 & 30.14 & 32.36 & 27.07 & 25.85 & 44.89 & 29.66  &  27.83\\
%         & LSSD & \textbf{14.49} & \textbf{21.5} & \textbf{31.66} & \textbf{33.57} & \textbf{28.37} & \textbf{26.95} & \textbf{46.21} & \textbf{31.07} & \textbf{29.23}\\
%         & $\Delta$ & +1.38 & +1.93 & +1.52 & +1.21 & +1.30 & +1.10 & +1.32 & +1.41 & +1.40\\
%         \midrule
        
%         \multirow{3}{*}{O2M} & \textsc{Baseline} & 7.40 & 13.09 & 25.71 & 25.66 & 16.93 & 20.94 & 41.68 & 23.35  &  21.85\\
%         & LSSD & \textbf{7.72} & \textbf{13.63} & \textbf{25.91} & \textbf{26.34} & \textbf{17.25} & \textbf{21.44} & \textbf{41.80}& \textbf{23.50} & \textbf{22.20} \\
%         & $\Delta$ & +0.32 & +0.54 & +0.20 & +0.68 & +0.32 & +0.50 & +0.12 & +0.15 & +0.35 \\
%     \bottomrule
%     \end{tabular}
%     \caption{BLEU scores of the baseline and LSSD on the test set of TED-8-Related dataset. Bold values indicate the best performance for each language pair. The left four languages are low-resource, and the right four languages are high-resource.}
%     \label{tab:related results}
%     \vspace{-3mm}
% \end{table*}

==> Unifying the Convergences in Multilingual Neural Machine Translation (Camera-Ready)/tables/single_teacher_results.tex <==
\begin{table}[t]
\small
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|cc|cc|cc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textsc{Diverse}} & \multicolumn{2}{c|}{\textsc{Related}} & \multicolumn{2}{c}{\textsc{WMT}} \\

& \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} \\
\midrule

% 29.00 22.85 27.83 21.85 20.15 19.07
LSSD &\textbf{+1.57} & \textbf{+0.70} & \textbf{+1.45} & \textbf{+0.35} & \textbf{+0.90} & \textbf{+0.69} \\

STSD & +0.89 & +0.00 & +0.86 & -0.14 & +0.18 & -0.20 \\
\bottomrule
\end{tabular}
\caption{BLEU score improvements of LSSD (Language-Specific Self-Distillation) and STSD (Single-Teacher Self-Distillation) over the \textsc{Multilingual} baseline on all three datasets.}
\label{tab:multiple teachers vs. single teacher.}
\end{table}

==> tables/DUB_results.tex <==
\begin{table}[t]
\small
\renewcommand\tabcolsep{2.0pt}
\centering
\begin{tabular}{l|cc|cc|cc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textsc{Diverse}} & \multicolumn{2}{c|}{\textsc{Related}} & \multicolumn{2}{c}{\textsc{WMT}} \\
& \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} & \textbf{M2O} & \textbf{O2M} \\
\midrule

\textsc{Multilingual} & 0.27 & 0.64 & 0.57 & 0.51 & 0.75 & 1.09\\

LSSD & 0.21 & 0.15 & 0.32 & 0.30 & 0.25 & 0.32 \\

$\Delta$ & $\downarrow$22\% & $\downarrow$77\% & $\downarrow$44\% & $\downarrow$41\% & $\downarrow$67\% & $\downarrow$71\% \\
\bottomrule
\end{tabular}
\caption{\textbf{DUB} (Distance to Upper-Bound) of the baselines and LSSD on all datasets.}
\label{tab:distance to upper bound in all datsets and settings.}
\end{table}

==> tables/results_WMT.tex <==

\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccc |c}
    \toprule
        & \textbf{Method} & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr} & \textbf{Avg.} \\
    \midrule
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -0.84 & -1.40 & +0.10 & +0.78 & \textbf{+0.71} & \textbf+0.82 & +0.03 \\
        
        & LSSD & \textbf{+0.64} & \textbf{+1.25} & \textbf{+1.58} & \textbf{+0.8} & +0.7 & \textbf{+1.1} & \textbf{+1.02} \\
        \midrule
        
        \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -2.42 & -2.26 & -0.69 & +0.58 & \textbf{+0.87} & \textbf{+0.92}  & -0.50 \\
        
        & LSSD & \textbf{+0.81} & \textbf{+0.53} & \textbf{+0.48} & \textbf{+1.0} & +0.68 & +0.66 & \textbf{+0.69} \\
    \bottomrule
    \end{tabular}
    \caption{BLEU scores improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline on the \textbf{WMT} dataset.
    We take the \textsc{LSSD-Selective} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold values indicate the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:WMT results}
    \vspace{-3mm}
\end{table*}

% \begin{table*}[th]
% \renewcommand\tabcolsep{3.5pt} 
% \small
%     \centering
%     \begin{tabular}{l | ccccccc | ccccccc}
%     \toprule
%         \multirow{2}{*}{Method} & \multicolumn{7}{c|}{\textbf{\textsc{Many-to-One}}} & \multicolumn{7}{c}{\textbf{\textsc{One-to-Many}}} \\ 
%         & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr} & \textbf{Avg.} 
%         & \textbf{Tr} & \textbf{Ro} & \textbf{Et} & \textbf{Zh} & \textbf{De} & \textbf{Fr} & \textbf{Avg.} \\
%         \midrule
        
%         \textsc{Multilingual} & 9.89 & 23.12 & 16.92 & 12.72 & 26.68 & 31.57 & 20.15 
%         & 8.83 & 18.42 & 13.34 & 20.78 & 21.11 & 31.93 & 19.07 \\
        
%         \textsc{Multi-Distill} & 9.05 & 21.72 & 17.02 & 13.50 & \textbf{27.39} & 32.39 & 20.18 
%         & 6.41 & 16.16 & 12.65 & 21.36 & \textbf{21.98} & 32.85 & 18.57 \\
%         \midrule
        
%         \textsc{LSSD-Whole} & \textbf{10.62} &\textbf{ 24.76} & 18.37 & 12.99 & 27.26 & 32.32 & 21.05 
%         & 9.47 & \textbf{18.85} & \textbf{13.85} & \textbf{21.38} & 21.87 & \textbf{32.98} & \textbf{19.73} \\
        
%         \textsc{LSSD-Select} & 10.53 & 24.37 & \textbf{18.50} & \textbf{13.52} & 27.38 & \textbf{32.67} & \textbf{21.17} 
%         & 9.05 & 18.44 & 13.52 & 20.98 & 21.58 & 32.32 & 19.32 \\
        
%         \textsc{LSSD-Adapt} & 10.39 & 24.63 & 18.18 & 13.19 & 27.01 & 32.08 & 20.91 
%         & \textbf{9.51} & 18.73 & 13.47 & 21.16 & 21.45 & 32.56 & 19.48 \\
%     \bottomrule
%     \end{tabular}
%     \caption{BLEU scores of two baselines and our LSSD on the WMT dataset. 
%     Languages are ordered increasingly by data size from left to right. 
%     \textbf{Bold} indicates the highest value.}
%     \label{tab:WMT results}
%     \vspace{-3mm}
% \end{table*}

==> tables/results_diverse.tex <==
%====================Diverse results
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccccc |c}
    \toprule
        & \textbf{Method} & \textbf{bos} & \textbf{mar} & \textbf{hin} & \textbf{mkd} & \textbf{ell} & \textbf{bul} & \textbf{fra}   & \textbf{kor} & \textbf{Avg.} \\
    \midrule
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -0.76 & -0.39 & -0.86 & +0.58 & +1.65 & +1.23 & +1.30 & +1.36 & +0.52 \\
        
        & LSSD & \textbf{+1.98} & \textbf{+1.00} & \textbf{+1.30} & \textbf{+2.17} & \textbf{+2.24} & \textbf{+1.81} & \textbf{+1.54} & \textbf{+2.10} & \textbf{+1.77} \\
        \midrule
        
        \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -3.44 & -0.87 & -1.26 & +0.41 & +0.49 & +0.35 & \textbf{+0.06} & -0.04  & -0.54 \\
        
        & LSSD & \textbf{+0.93} & \textbf{+0.37} & \textbf{+0.52} & \textbf{+2.37} & \textbf{+0.75} & \textbf{+0.39} & +0.04 & \textbf{+0.20} & \textbf{+0.70} \\
    \bottomrule
    \end{tabular}
    \caption{BLEU scores improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline on the \textbf{TED-8-Diverse} dataset.
    We take the \textsc{LSSD-Adaptive} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold values indicate the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:diverse results}
    \vspace{-3mm}
\end{table*}
%====================Diverse results Finished

% old version
% \begin{table*}[t]
% \small
%     \centering
%     \begin{tabular}{l|l | cccccccc |c}
%     \toprule
%         & \textbf{Method} & \textbf{bos} & \textbf{mar} & \textbf{hin} & \textbf{mkd} & \textbf{ell} & \textbf{bul} & \textbf{fra}   & \textbf{kor} & \textbf{Avg.} \\
%     \midrule
%         \multirow{3}{*}{M2O} & \textsc{Baseline} & 25.78 & 11.25 & 24.30 & 33.38 & 38.40 & 39.34 & 40.43 & 19.15  &  29.00\\
%         & LSSD & \textbf{27.33} & \textbf{12.34} & \textbf{24.87} & \textbf{35.37} & \textbf{40.12} & \textbf{41.41} & \textbf{42.04} & \textbf{21.24} & \textbf{30.59}\\
%         & $\Delta$ & +1.55 & +1.09 & +0.57 & +1.99 & +1.72 & +2.07 & +1.61 & +2.09 & +1.59 \\
%         \midrule
        
%         \multirow{3}{*}{O2M} & \textsc{Baseline} & 17.04 & 4.96 & 15.99 & 25.34 & 33.27 & 36.31 & 40.81 & 9.08  & 22.85 \\
%         & LSSD & \textbf{17.97} & \textbf{5.33} & \textbf{16.51} & \textbf{27.71} & \textbf{34.02} & \textbf{36.70} & \textbf{40.85} & \textbf{9.28} & \textbf{23.55} \\
%         & $\Delta$ & +0.93 & +0.37 & +0.52 & +2.37 & +0.75 & +0.39 & +0.04 & +0.20 & +0.70\\
%     \bottomrule
%     \end{tabular}
%     \caption{BLEU scores of the baseline and LSSD on the test set of TED-8-Diverse dataset. Bold values indicate the best performance for each language pair. Languages are ordered increasingly by data size from left to right.}
%     \label{tab:diverse results}
%     \vspace{-3mm}
% \end{table*}

==> tables/results_related.tex <==
%====================Related results
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|l | cccccccc | c}
    \toprule
        & \textbf{Method} & \textbf{aze} & \textbf{bel}	& \textbf{glg} & \textbf{slk} & \textbf{tur} & \textbf{rus} & \textbf{por} & \textbf{ces}	& \textbf{Avg.}\\
    \midrule
        \multirow{2}{*}{M2O} & \textsc{Multi-Distill} & -4.31 & -6.38 & -4.87 & +0.09 & \textbf{+1.52} & \textbf{+1.16} & \textbf{+1.62} & +1.33 & -1.23 \\
        & LSSD & \textbf{+1.53} & \textbf{+2.35} & \textbf{+1.7} & \textbf{+1.47} & +1.18 & +1.04 & +1.43 & \textbf{+1.82} & \textbf{+1.57}\\
        \midrule
        
        
        \multirow{2}{*}{O2M} & \textsc{Multi-Distill} & -5.57 & -10.89 & -5.54 & -1.10 & -0.54 & +0.33 & -0.26 & -1.17 & -3.10 \\
        & LSSD & \textbf{+0.37} & \textbf{+0.77} & \textbf{+0.69} & \textbf{+0.48} & \textbf{+0.36} & \textbf{+0.43} & \textbf{+0.04} & \textbf{+0.23} & \textbf{+0.42} \\
        
    \bottomrule
    \end{tabular}
    \caption{BLEU scores improvements of \textsc{Multi-Distill} and our LSSD over the \textsc{Multilingual} baseline on the \textbf{TED-8-Related} dataset. 
    We take the \textsc{LSSD-Adaptive} and \textsc{LSSD-Whole} as the representatives of LSSD in M2O and O2M translation respectively.
    Bold values indicate the best performance. 
    Languages are ordered increasingly by data size from left to right.}
    \label{tab:related results}
    \vspace{-3mm}
\end{table*}
%====================Related results Finished

% old version
% \begin{table*}[t]
% \small
%     \centering
%     \begin{tabular}{l|l | cccccccc | c}
%     \toprule
%         & \textbf{Method} & \textbf{aze} & \textbf{bel}	& \textbf{glg} & \textbf{slk} & \textbf{tur} & \textbf{rus} & \textbf{por} & \textbf{ces}	& \textbf{Avg.}\\
%     \midrule
%         \multirow{3}{*}{M2O} & \textsc{Baseline} & 13.11 & 19.57 & 30.14 & 32.36 & 27.07 & 25.85 & 44.89 & 29.66  &  27.83\\
%         & LSSD & \textbf{14.49} & \textbf{21.5} & \textbf{31.66} & \textbf{33.57} & \textbf{28.37} & \textbf{26.95} & \textbf{46.21} & \textbf{31.07} & \textbf{29.23}\\
%         & $\Delta$ & +1.38 & +1.93 & +1.52 & +1.21 & +1.30 & +1.10 & +1.32 & +1.41 & +1.40\\
%         \midrule
        
%         \multirow{3}{*}{O2M} & \textsc{Baseline} & 7.40 & 13.09 & 25.71 & 25.66 & 16.93 & 20.94 & 41.68 & 23.35  &  21.85\\
%         & LSSD & \textbf{7.72} & \textbf{13.63} & \textbf{25.91} & \textbf{26.34} & \textbf{17.25} & \textbf{21.44} & \textbf{41.80}& \textbf{23.50} & \textbf{22.20} \\
%         & $\Delta$ & +0.32 & +0.54 & +0.20 & +0.68 & +0.32 & +0.50 & +0.12 & +0.15 & +0.35 \\
%     \bottomrule
%     \end{tabular}
%     \caption{BLEU scores of the baseline and LSSD on the test set of TED-8-Related dataset. Bold values indicate the best performance for each language pair. The left four languages are low-resource, and the right four languages are high-resource.}
%     \label{tab:related results}
%     \vspace{-3mm}
% \end{table*}
